Adapted Large Language Models Can Outperform Medical Experts in Clinical Text Summarization

Analyzing vast textual data and summarizing key information from electronic health records imposes a substantial burden on how clinicians allocate their time. Although large language models (LLMs) have shown promise in natural language processing (NLP), their effectiveness on a diverse range of clinical summarization tasks remains unproven. In this study, we apply adaptation methods to eight LLMs, spanning four distinct clinical summarization tasks: radiology reports, patient questions, progress notes, and doctor-patient dialogue. Quantitative assessments with syntactic, semantic, and conceptual NLP metrics reveal trade-offs between models and adaptation methods. A clinical reader study with ten physicians evaluates summary completeness, correctness, and conciseness; in a majority of cases, summaries from our best adapted LLMs are either equivalent (45%) or superior (36%) compared to summaries from medical experts. The ensuing safety analysis highlights challenges faced by both LLMs and medical experts, as we connect errors to potential medical harm and categorize types of fabricated information. Our research provides evidence of LLMs outperforming medical experts in clinical text summarization across multiple tasks. This suggests that integrating LLMs into clinical workflows could alleviate documentation burden, allowing clinicians to focus more on patient care.

==> figures/reader_study/freq_plot.tex <==
\begin{figure*}[b!]
    \centering
    \includegraphics[width = 1\textwidth]{figures/reader_study/freq_plot_.pdf}
    \caption{
    Distribution of reader scores for each summarization task across evaluated attributes (completeness, correctness, conciseness). Horizontal axes denote reader preference between GPT-4 and human summaries as measured by a five-point Likert scale. Vertical axes denote frequency count, with 900 total reports for each plot. GPT-4 summaries are more often preferred in terms of correctness and completeness. While the largest gain in correctness occurs on radiology reports, this introduces a trade-off with conciseness. See Figure~\ref{fig:reader-study-main} for overall scores.}
    \label{fig:freq-plot}
\end{figure*}

==> figures/reader_study/reader_study.tex <==
\begin{figure*}%[b!]
    \centering
    \includegraphics[width = 0.7\textwidth]{figures/reader_study/reader_study_.pdf}
    \caption{Clinical reader study. \underline{\smash{Top}}: Study design comparing the summarization of GPT-4 vs. that of human experts on three attributes: completeness, correctness, and conciseness. \underline{\smash{Bottom}}: Results. GPT-4 summaries are rated higher than human summaries on completeness for all three summarization tasks and on correctness overall. Radiology reports highlight a trade-off between correctness (better) and conciseness (worse) with GPT-4.
    Highlight colors correspond to a value's location on the color spectrum. Asterisks denote statistical significance by Wilcoxon signed-rank test, *p-value $< 0.05$, **p-value $\ll 0.001$.}
    \label{fig:reader-study-main}
\end{figure*}

==> figures/reader_study/reader_table_main.tex <==
\setlength{\tabcolsep}{6pt} % spacing b/w cols, default 6pt
\setlength{\extrarowheight}{1.5pt}

\begin{table*}
  {\caption{\red{this proxy table will not appear in actual paper. please disregard.}}}
\begin{center}

{\begin{tabular}{l|ccc}
  \hline
  \textbf{Task}
              & \textbf{Completeness} & \textbf{Correctness} & \textbf{Conciseness} \\
  \hline
  Radiology reports  & **\colorbox{d1_ra_q1}{3.9 $\pm$ 9.8} & **\colorbox{d1_ra_q2}{2.5 $\pm$ 7.2} & *\colorbox{d1_ra_q3}{-1.7 $\pm$ 8.3} \\ 

  Patient questions  & **\colorbox{d2_ra_q1}{3.1 $\pm$ 13.0} & *\colorbox{d2_ra_q2}{0.7 $\pm$ 5.6} & \colorbox{d2_ra_q3}{0.4 $\pm$ 5.4} \\ 

  Progress notes  & **\colorbox{d3_ra_q1}{5.4 $\pm$ 13.9} & \colorbox{d3_ra_q2}{0.5 $\pm$ 8.0} & \colorbox{d3_ra_q3}{0.6 $\pm$ 6.9} \\ 
\hline 
 Overall  & **\colorbox{d99_r99_q1}{4.2 $\pm$ 11.4} & **\colorbox{d99_r99_q2}{1.2 $\pm$ 6.3} & \colorbox{d99_r99_q3}{-0.2 $\pm$ 7.2} \\ 

\hline
\end{tabular}}
\end{center}
\end{table*}
